UDA-Bench: Revisiting Common Assumptions in Unsupervised Domain Adaptation Using a Standardized Framework

In this work, we take a deeper look into the diverse factors that influence the efficacy of modern unsupervised domain adaptation (UDA) methods using a large-scale, controlled empirical study. To facilitate our analysis, we first develop UDA-Bench, a novel PyTorch framework that standardizes training and evaluation for domain adaptation enabling fair comparisons across several UDA methods. Using UDA-Bench, our comprehensive empirical study into the impact of backbone architectures, unlabeled data quantity, and pre-training datasets reveals that: (i) the benefits of adaptation methods diminish with advanced backbones, (ii) current methods underutilize unlabeled data, and (iii) pre-training data significantly affects downstream adaptation in both supervised and self-supervised settings. In the context of unsupervised adaptation, these observations uncover several novel and surprising properties, while scientifically validating several others that were often considered empirical heuristics or practitioner intuitions in the absence of a standardized training and evaluation framework. The UDA-Bench framework and trained models are publicly available at https://github.com/ViLab-UCSD/UDABench_ECCV2024.

==> tables/arch_uda.tex <==
\begin{table*}[!tb]
    \centering
    \caption{}
    \label{tab:arch_domain_robustness}
    \begin{minipage}{0.45\textwidth}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}cccccc@{}}
        \toprule
        Model & RN50 & SwinV2 & ConvNext & ResMLP & DeiT \\
        \midrule
        & \multicolumn{5}{c}{DomainNet (R$\rightarrow$C)} \\
        \cmidrule(lr){2-6}
        Plain & 43.32 & 55.51 & 50.8 & 46.62 & 50.75 \\
        DANN & 47.51 & 56.17 & 53.84 & 48.75 & 52.36 \\ 
        CDAN & 49.38 & 59.61 & 57.42 & 52.69 & 55.9  \\ 
        MDD & 46.38 & 60.46 & 52.66 & 50.44 & 56.05  \\ 
        MCC & 0 & 0 & 0 & 0 & 0 \\ 
        ToAlign & 50.2 & 57.84 & 56.67 & 51.84 & 53.9 \\
        MemSAC & 51.46 & 59.41 & 56.81 & 52.27 & 55.49 \\ 
        AdaMatch & 47.49 & 0 & 52.88 & 50.3 & 55.92 \\
        \cmidrule(lr){2-6}
        \graycolor{Tgt. Sup.} & \graycolor{71.4} & \graycolor{80.62} & \graycolor{77.66} & \graycolor{75.32} & \graycolor{78.81}\\
        \midrule
    \end{tabular}
    }
    \end{minipage}
\end{table*}

==> tables/batchnorm_plain.tex <==
% \begin{table*}[!tbhp]
%     \centering
%     \caption{Comparison of domain robustness of various vision architectures on standard adaptation datasets. We show the source accuracy ($\lambda_s$) and the target accuracy ($\lambda_t$) of a model trained only on source data, along with the relative drop in accuracy calculated as ($100*(\lambda_s-\lambda_t)/\lambda_s$). SWIN transformer has the best robustness to domain shifts.}
%     \label{tab:accuracy_comparison}
%     \begin{minipage}{\textwidth}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{@{}cccccc@{}}
%         \toprule
%         Model & ResNet-50~\cite{he2015deep} & Swin-V2-t~\cite{liu2022swin} & ConvNext-t~\cite{liu2022convnet} & ResMLP-s24~\cite{touvron2022resmlp} & \deit3-s~\cite{touvron2022deitiii} \\
%         \graycolor{\#Params} & \graycolor{24.12 M} & \graycolor{27.86 M} & \graycolor{28.10 M} & \graycolor{29.82 M} & \graycolor{21.86 M} \\
%         \midrule
%         %
%         & \multicolumn{5}{c}{DomainNet (R$\rightarrow$C)} \\
%         \cmidrule(lr){2-6}
%         Source Accuracy & 81.86/94.36 & 85.99/96.27 &  84.37/95.77 &  82.68/94.91 &  84.52/95.61 \\
%         Target Accuracy & 44.85/65.34 & 55.51/74.97 &  50.80/69.84 &  46.62/66.36 &  50.75/69.54 \\
%         \cmidrule(lr){2-6}
%         Rel. Drop (\%) ($\downarrow$) & 45.21/30.75 & \textbf{35.45}/\textbf{22.13} &  \underline{39.78}/\underline{27.08} &  43.61/30.09 &  39.95/27.27 \\
%         \midrule
%         %
%         & \multicolumn{5}{c}{\review{OfficeHome} (Re$\rightarrow$Ar)} \\
%         \cmidrule(lr){2-6}
%         Source Accuracy & 80.00/95.13 &  87.44/97.69 &  89.23/97.69 &  85.39/96.92 &  87.69/98.46 \\
%         Target Accuracy & 55.18/75.91 &  69.95/86.27 &  67.10/82.38 &  59.33/83.94 &  65.03/84.72 \\
%         \cmidrule(lr){2-6}
%         Rel. Drop (\%) ($\downarrow$) & 31.02/20.21 &  \textbf{20.00}/\textbf{11.69} &  \underline{24.80}/15.67 &  30.52/\underline{13.40} &  25.85/13.96 \\
%         \midrule
%         %
%         & \multicolumn{5}{c}{CUB200 (CUB$\rightarrow$Draw)} \\
%         \cmidrule(lr){2-6}
%         Source Accuracy & 81.00/96.00 &  87.75/98.38 &  85.88/97.38 &  84.62/96.62 &  88.12/97.75 \\
%         Target Accuracy & 52.60/74.10 &  58.90/81.53 &  49.53/73.76 &  53.41/75.90 &  56.36/76.17 \\
%         \cmidrule(lr){2-6}
%         Rel. Drop (\%) ($\downarrow$) & 35.06/22.81 &  \textbf{32.88}/\textbf{17.13} &  42.32/24.25 &  36.88/21.44 &  \underline{36.05}/\underline{22.08} \\
%         \midrule
%         %
%     \end{tabular}
%     }
%     \end{minipage}
% \end{table*}

\begin{table*}[!tb]
    \centering
    \caption{{\bf Effect of target normalization on unsupervised adaptation} We show that just updating batch statistics using target mini-batch during training already yields non-trivial accuracy gains over a source-only trained baseline model. While unsupervised adaptation methods do offer complimentary benefits, the actual gains offered are significantly lesser. $\lambda_o$ is the baseline accuracy, $\lambda_b$ is the accuracy when target mini-batch is used in normalization layers, $\lambda_M$ is the accuracy after adaptation using $M$, and $\sigma_M$ is the marginal benefit offered by $M$ alone. }
    \label{tab:arch_domain_robustness}
    \begin{minipage}{0.9\textwidth}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}ccccccc@{}}
        \toprule
        & RN50 & SwinV2 & ConvNext & ResMLP & DeiT & Avg. \\
        \midrule
        %
        & \multicolumn{6}{c}{DomainNet (S$\rightarrow$P)} \\
        \cmidrule(lr){2-7}
        Plain ($\lambda_o$) & 33.35 & 43.53 & 43.28 & 40.04 & 42.08 & 40.45  \\
        Plain + tgt. mini-batch ($\lambda_b$) & 40.47 & 47.32 & 47.39 & 43.34 & 45.21 & 44.74  \\
        \addlinespace[0.5em]
        $\lambda_{\text{MemSAC}}$ ($\sigma_{\text{MemSAC}}$) & 46.32 (0.55) & 52.50 (0.42) & 53.96 (0.38) & 48.90 (0.37) & 50.06 (0.39) & 50.34 (0.42) \\
        % \cline{1-6}
        $\lambda_{\text{AdaMatch}}$ ($\sigma_{\text{AdaMatch}}$) & 42.88 (0.75) & 50.50 (0.54) & 48.89 (0.73) & 44.48 (0.74) & 48.43 (0.49) & 47.03 (0.65) \\
        $\lambda_{\text{CDAN}}$ ($\sigma_{\text{CDAN}}$) & 40.80 (0.96) & 51.80 (0.46) & 52.00 (0.47) & 47.11 (0.47) & 48.93 (0.46) & 48.12 (0.56) \\
        \midrule
        %
        % & \multicolumn{6}{c}{CUB200 (C$\rightarrow$D)} \\
        % \cmidrule(lr){2-7}
        % Plain ($\lambda_o$) & 33.35 & 43.53 & 43.28 & 40.04 & 42.08 & 40.45  \\
        % Plain + tgt. mini-batch ($\lambda_b$) & 40.47 & 47.32 & 47.39 & 43.34 & 45.21 & 44.74  \\
        % \addlinespace[0.5em]
        % $\lambda_{\text{MemSAC}}$ ($\sigma_{\text{MemSAC}}$) & 46.32 (0.55) & 52.50 (0.42) & 53.96 (0.38) & 48.90 (0.37) & 50.06 (0.39) & 50.34 (0.42) \\
        % % \cline{1-6}
        % $\lambda_{\text{AdaMatch}}$ ($\sigma_{\text{AdaMatch}}$) & 42.88 (0.75) & 50.50 (0.54) & 48.89 (0.73) & 44.48 (0.74) & 48.43 (0.49) & 47.03 (0.65) \\
        % $\lambda_{\text{CDAN}}$ ($\sigma_{\text{CDAN}}$) & 40.80 (0.96) & 51.80 (0.46) & 52.00 (0.47) & 47.11 (0.47) & 48.93 (0.46) & 48.12 (0.56) \\
        %
    \end{tabular}
    }
    \end{minipage}
\end{table*}


==> tables/pretraining_table.tex <==
\begin{table*}
    \caption{Does pre-training domain matter for UDA?}
  \begin{minipage}[t]{0.43\textwidth}
    \centering
    \subcaption{Source-only training}
    \label{tab:pre-training}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lccc}
      % \toprule
      Pretraining & DNet & GeoP & CUB \\
      \midrule
      \multicolumn{4}{c}{Source-Only} \\
      \midrule
      ILSVRC-1M & 41.46 & 34.55 & 50.2 \\
      Places205-1M & 35.14 & 41.95 & 40.83 \\
      iNat2021-1M & 33.77 & 31.53 & 58.77 \\
      % \bottomrule
      % \bottomrule
      % \multicolumn{4}{c}{CDAN}
      % \midrule
      % ILSVRC-1M & 47.9 & 32.46 & 61.04 \\
      % Places205-1M & 39.54 & 39.19 & 49.13 \\
      % iNat2021-1M & 37.38 & 29.26 & 63.59 \\
      \bottomrule
      \bottomrule
      \multicolumn{4}{c}{MemSAC} \\
      \midrule
      ILSVRC-1M & 50.75 & 32.98 & 62.92 \\
      Places205-1M & 41.93 & 40.16 & 54.22 \\
      iNat2021-1M & 38.67 & 29.99 & 67.34 \\
    \end{tabular}
    }
    %%%%
  \end{minipage}\hfill
  \begin{minipage}[t]{0.43\textwidth}
    \centering
    \subcaption{Source-only training}
    \label{tab:pre-training}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lccc}
      % \toprule
      Pretraining & DNet & GeoP & CUB \\
      \midrule
      \multicolumn{4}{c}{Source-Only} \\
      \midrule
      ILSVRC-1M & 36.51 & 35.76 & 31.59 \\
      Places205-1M & 30.86 & 42.26 & 27.44 \\
      iNat2021-1M & 28.01 & 29.01 & 30.12 \\
      \bottomrule
      \bottomrule
      % \multicolumn{4}{c}{CDAN}
      % \midrule
      % ILSVRC-1M & 42.51 & 32.92 & 44.71 \\
      % Places205-1M & 35.3 & 38.36 & 32.93 \\
      % iNat2021-1M & 30.66 & 28.46 & 40.7 \\
      % \bottomrule
      % \bottomrule
      \multicolumn{4}{c}{MemSAC} \\
      \midrule
      ILSVRC-1M & 44.6 & 36.33 & 51.81 \\
      Places205-1M & 36.48 & 41.14 & 39.49 \\
      iNat2021-1M & 31.6 & 28.75 & 45.65 \\
    \end{tabular}
    }
  \end{minipage}\hfill
  %%%%
  %%%%%
  %%%%
  % \begin{minipage}[t]{0.23\textwidth}
  %   \centering
  %   \subcaption{Source-only training}
  %   \label{tab:pre-training}
  %   \resizebox{\textwidth}{!}{%
  %   \begin{tabular}{lccc}
  %     % \toprule
  %     Pretraining & DNet & GeoP & CUB \\
  %     \midrule
  %     \multicolumn{4}{c}{Source-Only} \\
  %     \midrule
  %     ILSVRC-1M & 41.46 & 34.55 & 50.2 \\
  %     Places205-1M & 35.14 & 41.95 & 40.83 \\
  %     iNat2021-1M & 33.77 & 31.53 & 58.77 \\
  %     % \bottomrule
  %     % \bottomrule
  %     % \multicolumn{4}{c}{CDAN}
  %     % \midrule
  %     % ILSVRC-1M & 47.9 & 32.46 & 61.04 \\
  %     % Places205-1M & 39.54 & 39.19 & 49.13 \\
  %     % iNat2021-1M & 37.38 & 29.26 & 63.59 \\
  %     \bottomrule
  %     \bottomrule
  %     \multicolumn{4}{c}{MemSAC} \\
  %     \midrule
  %     ILSVRC-1M & 50.75 & 32.98 & 62.92 \\
  %     Places205-1M & 41.93 & 40.16 & 54.22 \\
  %     iNat2021-1M & 38.67 & 29.99 & 67.34 \\
  %   \end{tabular}
  %   }
  %   %%%%
  % \end{minipage}\hfill
  % \begin{minipage}[t]{0.23\textwidth}
  %   \centering
  %   \subcaption{Source-only training}
  %   \label{tab:pre-training}
  %   \resizebox{\textwidth}{!}{%
  %   \begin{tabular}{lccc}
  %     % \toprule
  %     Pretraining & DNet & GeoP & CUB \\
  %     \midrule
  %     \multicolumn{4}{c}{Source-Only} \\
  %     \midrule
  %     ILSVRC-1M & 36.51 & 35.76 & 31.59 \\
  %     Places205-1M & 30.86 & 42.26 & 27.44 \\
  %     iNat2021-1M & 28.01 & 29.01 & 30.12 \\
  %     \bottomrule
  %     \bottomrule
  %     % \multicolumn{4}{c}{CDAN}
  %     % \midrule
  %     % ILSVRC-1M & 42.51 & 32.92 & 44.71 \\
  %     % Places205-1M & 35.3 & 38.36 & 32.93 \\
  %     % iNat2021-1M & 30.66 & 28.46 & 40.7 \\
  %     % \bottomrule
  %     % \bottomrule
  %     \multicolumn{4}{c}{MemSAC} \\
  %     \midrule
  %     ILSVRC-1M & 44.6 & 36.33 & 51.81 \\
  %     Places205-1M & 36.48 & 41.14 & 39.49 \\
  %     iNat2021-1M & 31.6 & 28.75 & 45.65 \\
  %   \end{tabular}
  %   }
  % \end{minipage}\hfill
  %%%%
\end{table*}


==> tables/pt_supervised_daln.tex <==
\begin{table*}[b]
\centering
    \captionsetup{width=0.7\textwidth, font=footnotesize}
    \caption{{\bf Additional result for the pre-training experiment on DALN} In addition to the Table 2 in the paper, we show that the benefits conferred by in-domain pre-training also hold for various UDA methods, as shown for the case of DALN.}
  \begin{minipage}[t]{0.48\textwidth}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c cccc}
    \toprule
       && \multicolumn{3}{c}{DALN} \\
      \cmidrule{3-5}
      Pre-training && DNet & GeoP & CUB \\
      % \midrule
      \cmidrule{1-1} \cmidrule{3-5} 
      ILSVRC-1M && \textbf{47.59} & 26.85 & 61.45   \\
      Places205-1M && 39.21 & \textbf{36.23} & 50.74  \\
      iNat2021-1M && 37.30 & 24.69 & \textbf{66.80} \\
      \bottomrule
    \end{tabular}
    }
  \end{minipage}
\end{table*}

